Generative Diffusion Prior for Unified Image Restoration and Enhancement

Existing image restoration methods mostly leverage the posterior distribution of natural images. However, they often assume known degradation and also require supervised training, which restricts their adaptation to complex real applications. In this work, we propose the Generative Diffusion Prior (GDP) to effectively model the posterior distributions in an unsupervised sampling manner. GDP utilizes a pre-train denoising diffusion generative model (DDPM) for solving linear inverse, non-linear, or blind problems. Specifically, GDP systematically explores a protocol of conditional guidance, which is verified more practical than the commonly used guidance way. Furthermore, GDP is strength at optimizing the parameters of degradation model during the denoising process, achieving blind image restoration. Besides, we devise hierarchical guidance and patch-based methods, enabling the GDP to generate images of arbitrary resolutions. Experimentally, we demonstrate GDP's versatility on several image datasets for linear problems, such as super-resolution, deblurring, inpainting, and colorization, as well as non-linear and blind issues, such as low-light enhancement and HDR image recovery. GDP outperforms the current leading unsupervised methods on the diverse benchmarks in reconstruction quality and perceptual quality. Moreover, GDP also generalizes well for natural images or synthesized images with arbitrary sizes from various tasks out of the distribution of the ImageNet training set.

==> latex/algos/algo1_bak.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[t]\footnotesize
	\caption{GDP-$x_t$: Conditioner guided diffusion sampling on $\boldsymbol{x}_{t}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, conditioner $p_{\theta}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right)$.}
	\KwIn{Corrupted image $\boldsymbol{y}$, gradient scale $s$, known degradation model $\mathcal{D}$}
	\KwOut{$\boldsymbol{x}_{T} \leftarrow$ sample from $\mathcal{N}(0, \mathbf{I})$}
	\For{all $t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
	    
	    $\nabla_{\boldsymbol{x}_{t}} \log p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right) \leftarrow -\nabla_{\boldsymbol{x}_{t}} \mathcal{L}\left(\boldsymbol{y}, \mathcal{D}\left(\boldsymbol{x}_{t}\right)\right)$\\

		$\boldsymbol{x}_{t-1} \leftarrow$ sample from $\mathcal{N}\left(\mu+s \nabla_{\boldsymbol{x}_{t}} \log p_{\theta}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right), \Sigma\right)$
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo1}
\end{algorithm}

==> latex/algos/algo1_bak1.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[t]\footnotesize
	\caption{\textbf{GDP-}$\boldsymbol{x}_t$: Conditioner guided diffusion sampling on $\boldsymbol{x}_{t}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, corrupted image conditioner $\boldsymbol{y}$. 
 % \lyu{why alg 1 has known degradation and alg2 has unknown.}
 }
	\KwIn{Corrupted image $\boldsymbol{y}$, gradient scale $s$, degradation model $\mathcal{D}_\phi$ with randomly initiated parameters $\phi$, learning rate $l$ for optimizable degradation model, distance measure $\mathcal{L}$.}
	\KwOut{Output image $\boldsymbol{x}_{0}$ conditioned on $\boldsymbol{y}$}
        Sample $\boldsymbol{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
        
	\For{all $t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    % $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
        $\phi \leftarrow \phi - l \nabla_{\phi} \mathcal{L}(\boldsymbol{y}, {\mathcal{D}_\phi}\left(\boldsymbol{{x}}_{t}\right))$
    
	   $\boldsymbol{{x}}_{t} \leftarrow \boldsymbol{x}_{t} -s\nabla_{\boldsymbol{{x}}_{t}} \mathcal{L}\left(\boldsymbol{y}, {\mathcal{D}_{\phi}}\left(\boldsymbol{x_{t}}\right)\right)$ \\
	    % $\nabla_{\boldsymbol{x}_{t}} \log p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right) \leftarrow -\nabla_{\boldsymbol{x}_{t}} \mathcal{L}\left(\boldsymbol{y}, \mathcal{D}\left(\boldsymbol{x}_{t}\right)\right)$\\

		% $\boldsymbol{x}_{t-1} \leftarrow$ sample from $\mathcal{N}\left(\mu+s \nabla_{\boldsymbol{x}_{t}} \log p_{\theta}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right), \Sigma\right)$
  
        Sample $\boldsymbol{x}_{t-1}$ by $q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_{t}\right)=\mathcal{N}\left(\boldsymbol{x}_{t}; \sqrt{1-\beta_t} \boldsymbol{x}_{t-1}, \beta_t \mathbf{I}\right)$,
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo1}
\end{algorithm}

==> latex/algos/algo2_bak.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[htbp]  
	\caption{\textbf{GDP-$\boldsymbol{x}_0$}: Conditioner guided diffusion sampling on $\boldsymbol{x}_{0}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, conditioner $p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right)$.}
	\KwIn{degraded image $\boldsymbol{y}$, gradient scale $s$, degradation model $\mathcal{D}_\theta$ with randomly initiated parameters.}
	\KwOut{$\boldsymbol{x}_{T} \leftarrow$ sample from $\mathcal{N}(0, \mathbf{I})$}
	\For{all $t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
	    
	    $\boldsymbol{\tilde{x}}_{0} =  \frac{\boldsymbol{x}_{t}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$

	    $\boldsymbol{\widehat{x}}_{0} = {\mathcal{D}_\theta}\left(\boldsymbol{\tilde{x}}_{0}\right)$
	    
	    $\nabla_{\boldsymbol{\widehat{x}}_{0}} \log p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{\widehat{x}}_{0}\right) = -\nabla_{\boldsymbol{x}_{t}} \mathcal{L}\left(\boldsymbol{y}, \left(\boldsymbol{\widehat{x}}_{0}\right)\right)$\\

       $\theta = \theta - l \nabla_{\theta} \mathcal{L}(\boldsymbol{y}, \boldsymbol{\widehat{x}}_{0})$
		
		$\boldsymbol{x}_{t-1} \leftarrow$ sample from $\mathcal{N}\left(\mu+s  \nabla_{\boldsymbol{\widehat{x}}_{0}} \log p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{\widehat{x}}_{0}\right), \Sigma\right)$
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo2}
\end{algorithm}

==> latex/algos/algo2_bak1.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[t]\footnotesize
	\caption{\textbf{GDP-$\boldsymbol{x}_0$}: Conditioner guided diffusion sampling on $\boldsymbol{\tilde{x}}_{0}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, corrupted image conditioner $\boldsymbol{y}$.}
	\KwIn{Corrupted image $\boldsymbol{y}$, gradient scale $s$, degradation model $\mathcal{D}_\phi$ with randomly initiated parameters $\phi$, learning rate $l$ for optimizable degradation model, distance measure $\mathcal{L}$.}
	\KwOut{Output image $\boldsymbol{x}_{0}$ conditioned on $\boldsymbol{y}$}
        Sample $\boldsymbol{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
        
	\For{$t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    % $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
	    
	    $\boldsymbol{\tilde{x}}_{0} =  \frac{\boldsymbol{x}_{t}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$

	    % $\boldsymbol{\widehat{x}}_{0} = {\mathcal{D}_\theta}\left(\boldsymbol{\tilde{x}}_{0}\right)$

        $\phi \leftarrow \phi - l \nabla_{\phi} \mathcal{L}(\boldsymbol{y}, {\mathcal{D}_\phi}\left(\boldsymbol{\tilde{x}}_{0}\right))$
            
	    $\boldsymbol{\tilde{x}}_{0} \leftarrow \boldsymbol{\tilde{x}}_{0} -s\nabla_{\boldsymbol{\tilde{x}}_{0}} \mathcal{L}\left(\boldsymbol{y}, \left({\mathcal{D}_\phi}\left(\boldsymbol{\tilde{x}}_{0}\right)\right)\right)$\\


		
		% $\boldsymbol{x}_{t-1} \leftarrow$ sample from $\mathcal{N}\left(\mu+s  \nabla_{\boldsymbol{\widehat{x}}_{0}} \log p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{\widehat{x}}_{0}\right), \Sigma\right)$
        Sample $\boldsymbol{x}_{t-1}$ by $q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_{t}, \boldsymbol{\tilde{x}}_{0}\right) =\mathcal{N}\left(\boldsymbol{x}_{t-1}; \tilde{\boldsymbol{\mu}}_t\left(\boldsymbol{x}_{t}, \boldsymbol{\tilde{x}}_{0}\right), \tilde{\beta}_t \mathbf{I}\right)$, 
        
        where $\quad \tilde{\boldsymbol{\mu}}_t\left(\boldsymbol{x}_{t}, \boldsymbol{\tilde{x}}_{0}\right)=\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} \boldsymbol{\tilde{x}}_{0}+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \boldsymbol{x}_{t} \quad$ and $\quad \tilde{\beta}_t=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo2}
\end{algorithm}

==> latex/algos/algo3.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[htbp]  
	\caption{\textbf{HDR-GDP-$\boldsymbol{x}_0$}: Conditioner guided diffusion sampling on $\boldsymbol{x}_{0}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, corrupted images conditioner $\{\boldsymbol{y}^n \mid n=3\}$.}
	\KwIn{LDR-long image $\boldsymbol{y}^1$, LDR-medium image $\boldsymbol{y}^2$, LDR-short image $\boldsymbol{y}^3$, gradient scale $s$, degradation model $\{\mathcal{D}^n_\phi  \mid n=3\}$ with randomly initiated parameters $\phi$, learning rate $l$ for optimizable degradation model, distance measure $\mathcal{L}$.}
	\KwOut{Output image $\boldsymbol{x}_{0}$ conditioned on $\{\boldsymbol{y}^n \mid n=3\}$}
        Sample $\boldsymbol{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
        
	\For{$t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    % $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
	    
	    $\boldsymbol{\tilde{x}}_{0} \leftarrow \frac{\boldsymbol{x}_{t}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$


        $\mathcal{L}_{total} = 0$
        
	    \For{$j$ from 1 to 3}{
     	    
     %      $\boldsymbol{\widehat{x}}_{0} = {\mathcal{D}^i_\theta}\left(\boldsymbol{\tilde{x}}_{0}\right)$
          
	    % $\nabla_{\boldsymbol{\widehat{x}}_{0}} \log p_{\phi}\left(\boldsymbol{y_i} \mid \boldsymbol{\widehat{x}}_{0}\right) = -\nabla_{\boldsymbol{x}_{t}} \mathcal{L}\left(\boldsymbol{y^i}, \left(\boldsymbol{\widehat{x}}_{0}\right)\right)$

     %       $\theta = \theta - l \nabla_{\theta} \mathcal{L}(\boldsymbol{y^j}, \boldsymbol{\widehat{x}}_{0})$
     %    $\phi = \phi - l \nabla_{\phi} \mathcal{L}\left(\boldsymbol{y}^j, {\mathcal{D}^j_\phi}\left(\boldsymbol{\tilde{x}}_{0}\right)\right)$
        
	    % $\boldsymbol{\tilde{x}}_{0}^j = \boldsymbol{\tilde{x}}_{0} -s\nabla_{\boldsymbol{\tilde{x}}_{0}} \mathcal{L}\left(\boldsymbol{y}^j, {\mathcal{D}^j_\phi}\left(\boldsymbol{\tilde{x}}_{0}\right)\right)$


        $\mathcal{L}_{total} = \mathcal{L}_{total} + \mathcal{L}\left(\boldsymbol{y}^j, {\mathcal{D}^j_\phi}\left(\boldsymbol{\tilde{x}}_{0}\right)\right) $
	    }

        $\phi = \phi - l \nabla_{\phi} \mathcal{L}_{total}$

        $\boldsymbol{\tilde{x}}_{0} = \boldsymbol{\tilde{x}}_{0} - s\nabla_{\boldsymbol{\tilde{x}}_{0}} \mathcal{L}_{total}$

        Sample $\boldsymbol{x}_{t-1}$ by $q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_{t}, \boldsymbol{\tilde{x}}_{0}\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1}; \tilde{\boldsymbol{\mu}}_t\left(\boldsymbol{x}_{t}, \boldsymbol{\tilde{x}}_{0}\right), \tilde{\beta}_t \mathbf{I}\right)$, 
        
        where $\quad \tilde{\boldsymbol{\mu}}_t\left(\boldsymbol{x}_{t}, \boldsymbol{\tilde{x}}_{0}\right)=\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} \boldsymbol{\tilde{x}}_{0}+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \boldsymbol{x}_{t} \quad$ and $\quad \tilde{\beta}_t=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$
        
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo3}
\end{algorithm}

==> latex/algos/algo4_bak.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[t]\footnotesize
	\caption{GDP-$x_0$: Conditioner guided diffusion sampling on $\boldsymbol{x}_{0}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, conditioner $p_{\phi}\left(\boldsymbol{y}^i \mid \boldsymbol{x}_{t}\right)$.}
	\KwIn{Corrupted image $\boldsymbol{y^i}$ ($i$ = 3 for HDR recovery and $i$ = 1 for other tasks), gradient scale $s$, degradation model $\mathcal{D}^i_\theta$ with randomly initiated parameters.}
	\KwOut{$\boldsymbol{x}_{T} \leftarrow$ sample from $\mathcal{N}(0, \mathbf{I})$}
	\For{all $t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
	    
	    $\boldsymbol{\tilde{x}}_{0}  =  \frac{\boldsymbol{x}_{t}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$
	    
	    \For{$j$ from 1 to i}{
	    $\boldsymbol{\widehat{x}}_{0} = {\mathcal{D}^j_\theta}\left(\boldsymbol{\tilde{x}}_{0}\right)$
	    
	    $\nabla_{\boldsymbol{\widehat{x}}_{0}} \log p_{\phi}\left(\boldsymbol{y^j} \mid \boldsymbol{\widehat{x}}_{0}\right) = -\nabla_{\boldsymbol{\widehat{x}}_{0}} \mathcal{L}\left(\boldsymbol{y^j}, \boldsymbol{\widehat{x}}_{0}\right)$
	    
	    % ${\mathcal{D}^j} \leftarrow -\nabla_{\mathcal{D}^j} \mathcal{L}\left(\boldsymbol{y^i}, \boldsymbol{\widehat{x}}_{0}\right)$
        $\theta = \theta - l \nabla_{\theta} \mathcal{L}(\boldsymbol{y^j}, \boldsymbol{\widehat{x}}_{0})$
	    }
	    
		$\boldsymbol{x}_{t-1} \leftarrow$ sample from $\mathcal{N}\left(\mu+ s \nabla_{\boldsymbol{\widehat{x}}_{0}} \log p_{\phi}\left(\boldsymbol{y^i} \mid \boldsymbol{\widehat{x}}_{0}\right), \Sigma \right)$
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo4}
\end{algorithm}

==> latex/algos/algo5_bak.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[t]\footnotesize
	\caption{\textbf{GDP-}$\boldsymbol{x}_t$ with fixed degradation model: Conditioner guided diffusion sampling on $\boldsymbol{x}_{t}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, corrupted image conditioner $\boldsymbol{y}$. 
 % \lyu{why alg 1 has known degradation and alg2 has unknown.}
 }
	\KwIn{Corrupted image $\boldsymbol{y}$, gradient scale $s$, degradation model $\mathcal{D}$, distance measure $\mathcal{L}$.}
	\KwOut{Output image $\boldsymbol{x}_{0}$ conditioned on $\boldsymbol{y}$}
        Sample $\boldsymbol{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
        
	\For{all $t$ from $T$ to 1}{
	    % $pcd\_map$ \leftarrow k\_mask(y, M(\boldsymbol{x}^{t}))\\
	    % $\mu, \Sigma \leftarrow \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
        % $\phi \leftarrow \phi - l \nabla_{\phi} \mathcal{L}(\boldsymbol{y}, {\mathcal{D}_\phi}\left(\boldsymbol{\tilde{x}}_{0}\right))$
    
	   $\boldsymbol{{x}}_{t} \leftarrow \boldsymbol{x}_{t} -s\nabla_{\boldsymbol{{x}}_{t}} \mathcal{L}\left(\boldsymbol{y}, {\mathcal{D}}\left(\boldsymbol{x_{t}}\right)\right)$ \\
	    % $\nabla_{\boldsymbol{x}_{t}} \log p_{\phi}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right) \leftarrow -\nabla_{\boldsymbol{x}_{t}} \mathcal{L}\left(\boldsymbol{y}, \mathcal{D}\left(\boldsymbol{x}_{t}\right)\right)$\\

		% $\boldsymbol{x}_{t-1} \leftarrow$ sample from $\mathcal{N}\left(\mu+s \nabla_{\boldsymbol{x}_{t}} \log p_{\theta}\left(\boldsymbol{y} \mid \boldsymbol{x}_{t}\right), \Sigma\right)$
  
        Sample $\boldsymbol{x}_{t-1}$ by $q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_{t}\right)=\mathcal{N}\left(\boldsymbol{x}_{t}; \sqrt{1-\beta_t} \boldsymbol{x}_{t-1}, \beta_t \mathbf{I}\right)$,
	}
	\Return $\boldsymbol{x}_{0}$
\label{algo5}
\end{algorithm}

==> latex/algos/patch-based.tex <==
% !TEX root = ../PaperForReview.tex

\begin{algorithm}[t]\footnotesize
    \caption{Restore Any-size Image}
    \KwIn{Conditioner guided diffusion sampling on $\boldsymbol{\tilde{x}}_{0}$, given a diffusion model $\left(\mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)\right)$, corrupted image conditioner $\boldsymbol{y}$ (We take a banner image for instance), optimizable degradation model $\mathcal{D}_{\phi^l}: \boldsymbol{\overline{y}}^l=f^l \boldsymbol{x}^l+\boldsymbol{\mathcal{\overline{M}}}^l$ and $\mathcal{D}_{\phi^r}: \boldsymbol{\overline{y}}^r=f^r \boldsymbol{x}^r+\boldsymbol{\mathcal{\overline{M}}}^r$ for left and right patches, respectively. Dictionary of $O$ overlapping patch locations.}
    \KwOut{Output image $\boldsymbol{x}_{0}$ conditioned on $\boldsymbol{y}$}

    Sample $\boldsymbol{x}_{T}$ from $\mathcal{N}(0, \mathbf{I})$
    
    \For{$t$ from $T$ to 1}{

    1: $\mu, \Sigma = \mu_{\theta}\left(\boldsymbol{x}_{t}\right), \Sigma_{\theta}\left(\boldsymbol{x}_{t}\right)$
    
    2: Resize $\boldsymbol{x}_{t}, \boldsymbol{y} \in \mathbb{R}^{3 \times H \times W} $ to $\boldsymbol{\overline{x}}_{t}, \boldsymbol{\overline{y}} \in \mathbb{R}^{3 \times 256 \times \overline{W}}$

    3: Crop the $\boldsymbol{\overline{y}}$ into left patch $\boldsymbol{\overline{y}}^l$ and right patch $\boldsymbol{\overline{y}}^r$; Crop the $\boldsymbol{\overline{x}}_{t}$ into left patch $\boldsymbol{\overline{x}}_{t}^l$ and right patch $\boldsymbol{\overline{x}}_{t}^r$
	    
    4: $\boldsymbol{\tilde{x}}_{0}^l  =  \frac{\boldsymbol{\overline{x}}_{t}^l}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$

    5: $\boldsymbol{\tilde{x}}_{0}^r  =  \frac{\boldsymbol{\overline{x}}_{t}^r}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$

    6: $\mathcal{L}^{l, total}_{{\phi^l}, \boldsymbol{\tilde{x}}_{0}^l} = \mathcal{L}(\boldsymbol{\overline{y}}^l, {\mathcal{D}_{\phi^l}}\left(\boldsymbol{\tilde{x}}_{0}^l\right)) + \frac{\lambda}{s}\mathcal{Q}\left(\boldsymbol{\tilde{x}}_{0}^l\right)$ 

    7: $\mathcal{L}^{r, total}_{{\phi^r}, \boldsymbol{\tilde{x}}_{0}^r} = \mathcal{L}(\boldsymbol{\overline{y}}^r, {\mathcal{D}_{\phi^r}}\left(\boldsymbol{\tilde{x}}_{0}^l\right)) + \frac{\lambda}{s}\mathcal{Q}\left(\boldsymbol{\tilde{x}}_{0}^r\right)$ 

    8: ${\phi^l} \leftarrow {\phi^l} - l \nabla_{\phi^l} \mathcal{L}^{l, total}_{{\phi^l}, \boldsymbol{\tilde{x}}_{0}^l}$

    9: ${\phi^r} \leftarrow {\phi^r} - l \nabla_{\phi^r} \mathcal{L}^{r, total}_{{\phi^r}, \boldsymbol{\tilde{x}}_{0}^r}$
            
    10: Sample $\boldsymbol{x}_{t-1}^l$ by $\mathcal{N}\left(\mu+s\nabla_{\boldsymbol{\tilde{x}}_{0}^l} \mathcal{L}^{l, total}_{{\phi^l}, \boldsymbol{\tilde{x}}_{0}^l}, \Sigma\right)$

    11: Sample $\boldsymbol{x}_{t-1}^r$ by $\mathcal{N}\left(\mu+s\nabla_{\boldsymbol{\tilde{x}}_{0}^r} \mathcal{L}^{r, total}_{{\phi^r}, \boldsymbol{\tilde{x}}_{0}^r}, \Sigma\right)$

    12: Grids $\overline{G}$ are initialized with the same shape as $\boldsymbol{\overline{y}}$

    13: $\overline{G}[:, :, 0:256, 0:256] += 1$ and $\overline{G}[:, :, {\overline{W}}-\text{patch size}, {\overline{W}}-\text{patch size}:256] += 1$

    14: $\boldsymbol{\overline{x}}_{t}[:, :, 0:256, 0:256] += \boldsymbol{x}_{t-1}^l$ and $\boldsymbol{\overline{x}}_{t}[:, :, {\overline{W}}-\text{patch size}, {\overline{W}}-\text{patch size}:256] += \boldsymbol{x}_{t-1}^r$

    15: $\boldsymbol{\mathcal{\overline{M}}}[:, :, 0:256, 0:256] += \boldsymbol{\mathcal{\overline{M}}}^l$ and $\boldsymbol{\overline{x}}_{t}[:, :, {\overline{W}}-\text{patch size}, {\overline{W}}-\text{patch size}:256] += \boldsymbol{\mathcal{\overline{M}}}^r$

    16: $\boldsymbol{\overline{x}}_{t} = \boldsymbol{\overline{x}}_{t} \oslash G$, $\boldsymbol{\mathcal{\overline{M}}} = \boldsymbol{\mathcal{\overline{M}}} \oslash G$, where $\oslash$ is element-wise division
    
    17: Interpolate $ \boldsymbol{\overline{x}}_{t}, \boldsymbol{\mathcal{\overline{M}}}$ into $\boldsymbol{x}_{t}, \boldsymbol{\mathcal{M}} \in \mathbb{R}^{3 \times H \times W}$

    18: $f = (f^l + f^r)/2$

    19: $G, \tilde{\mu}, \tilde{\Sigma} = 0, 0, 0$
    
    20: \For {$o = 1,\ldots,n$}{ 
    
        21: $\boldsymbol{x}_{t}^{(o)}=\operatorname{Crop}\left(\mathbf{P}_o \circ \boldsymbol{x}_{t}\right) \text { and } \boldsymbol{y}^{(o)}=\operatorname{Crop}\left(\mathbf{P}_o \circ \boldsymbol{y}\right) \text { and } \boldsymbol{\mathcal{M}}^{(o)}=\operatorname{Crop}\left(\mathbf{P}_o \circ \boldsymbol{\mathcal{M}}\right) \text { and } \mu^{(o)}=\operatorname{Crop}\left(\mathbf{P}_o \circ \mu^{(o)}\right) \text { and } \Sigma^{(o)}=\operatorname{Crop}\left(\mathbf{P}_o \circ \Sigma^{(o)}\right)$

        22: $\boldsymbol{\tilde{x}}^{(o)}_{0} =  \frac{\boldsymbol{x}^{(o)}_{t}}{\sqrt{\bar{\alpha}_{t}}}-\frac{\sqrt{1-\bar{\alpha}_{t}} \epsilon_{\theta}\left(\boldsymbol{x}^{(o)}_{t}, t\right)}{\sqrt{\bar{\alpha}_{t}}}$

        23: $\mathcal{L}^{total}_{ \boldsymbol{\tilde{x}}^{(o)}_{0}} = \mathcal{L}(\boldsymbol{y}^{(o)}, {\mathcal{D}}\left(\boldsymbol{\tilde{x}}^{(o)}_{0}\right)) + \frac{\lambda}{s}\mathcal{Q}\left(\boldsymbol{\tilde{x}}^{(o)}_{0}\right)$ 

        24: $\tilde{\mu} = \tilde{\mu} + \mathbf{P}_o \cdot \left(\mu^{(o)} + s\nabla_{\boldsymbol{\tilde{x}}^{(o)}_{0}} \mathcal{L}^{total}_{ \boldsymbol{\tilde{x}}^{(o)}_{0}}\right)$

        25: $\tilde{\Sigma} = \tilde{\Sigma} + \mathbf{P}_o \cdot \Sigma^{(o)}$

    }

    26: $G = G + \mathbf{P}_o $

    27: $\tilde{\Sigma} = \tilde{\Sigma} \oslash G$, $\tilde{\Sigma} = \tilde{\Sigma} \oslash G$
        
    28: Sample $\boldsymbol{x}_{t-1}$ by $\mathcal{N}\left(\tilde{\mu}, \tilde{\Sigma}\right)$
    }
        
    \Return Restored any-size image $\boldsymbol{x}_0$
\label{algo:patch}
\end{algorithm}
